Spectral analysis of high order continuous FEM for hyperbolic PDEs on triangular meshes: influence of approximation, stabilization, and time-stepping

In this work we study various continuous finite element discretization for two dimensional hyperbolic partial differential equations, varying the polynomial space (Lagrangian on equispaced, Lagrangian on quadrature points (Cubature) and Bernstein), the stabilization techniques (streamline-upwind Petrov-Galerkin, continuous interior penalty, orthogonal subscale stabilization) and the time discretization (Runge-Kutta (RK), strong stability preserving RK and deferred correction). This is an extension of the one dimensional study by Michel S. et al J. Sci. Comput. (2021), whose results do not hold in multi-dimensional frameworks. The study ranks these schemes based on efficiency (most of them are mass-matrix free), stability and dispersion error, providing the best CFL and stabilization coefficients. The challenges in two-dimensions are related to the Fourier analysis. Here, we perform it on two types of periodic triangular meshes varying the angle of the advection, and we combine all the results for a general stability analysis. Furthermore, we introduce additional high order viscosity to stabilize the discontinuities, in order to show how to use these methods for tests of practical interest. All the theoretical results are thoroughly validated numerically both on linear and non-linear problems, and error-CPU time curves are provided. Our final conclusions suggest that Cubature elements combined with SSPRK and OSS stabilization is the most promising combination.

==> CFL_TAU_tab_LinearAdvection_2D_meshT-RES.tex <==
\begin{table}[H] 
\small  
 \begin{center} 
		\begin{tabular}{| c | c || c | c | c | }  
	     \hline 
	     \multicolumn{2}{|c||}{Element $\&$ }  & \multicolumn{3}{|c|}{SUPG}  \\ \hline 
	     \multicolumn{2}{|c||}{ Time scheme }  & $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$  \\ \hline \hline 
       % lagrange basic 
        \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}}              &  SSPRK  &  0.739 (0.127)   &  0.403 (0.026)   &  0.298 (0.012)  \\ 
               &  RK  &  0.546 (0.058)   &  0.298 (0.026)   &  0.22 (0.012)  \\ 
         \hline 
       % lagrange cubature 
       \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}}              &  DeC  &  1.062 (0.127)   &  0.144 (0.078)   &  0.034 (0.153)  \\ 
               &  SSPRK  &  1.062 (0.28)   &  0.234 (0.078)   &  0.055 (0.153)  \\ 
               &  RK  &  1.062 (0.127)   &  0.144 (0.078)   &  0.034 (0.153)  \\ 
         \hline 
       % bernstein basic 
       \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}}              &  DeC  &  0.739 (0.298)   &  0.739 (0.153)   &  0.455 (0.153)  \\ 
               &  SSPRK  &  0.739 (0.127)   &  0.403 (0.026)   &  0.298 (0.012)  \\ 
               &  RK  &  0.546 (0.058)   &  0.298 (0.026)   &  0.22 (0.012)  \\ 
         \hline 
        \hline 
        \end{tabular} 
    \end{center} 
 \begin{center} 
		\begin{tabular}{| c | c || c | c | c || c | c | c | }  
	     \hline 
	     \multicolumn{2}{|c||}{Element $\&$ }  & \multicolumn{3}{|c||}{OSS}  & \multicolumn{3}{|c|}{CIP}  \\ \hline 
	     \multicolumn{2}{|c||}{ Time scheme }  & $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$   & $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$  \\ \hline \hline 
       % lagrange basic 
        \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Basic}}}              &  SSPRK  &  0.546 (0.127)   &  0.403 (0.058)   &  0.298 (0.012)   &  0.546 (0.026)   &  0.298 (7.39e-05)   &  0.298 (3.36e-05)   \\ 
               &  RK  &  0.298 (0.127)   &  0.298 (0.026)   &  0.22 (0.026)   &  0.403 (0.012)   &  0.298 (7.39e-05)   &  0.22 (3.36e-05)   \\ 
         \hline 
       % lagrange cubature 
       \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}}              &  DeC  &  0.58 (0.207)   &  0.379 (0.03)   &  /   &  0.58 (0.026)   &  0.045 (7.85e-03)   &   /   \\ 
               &  SSPRK  &  0.886 (0.336)   &  0.379 (0.048)   &  /   &  0.886 (0.048)   &  0.106 (7.85e-03)   &   /   \\ 
               &  RK  &  0.58 (0.207)   &  0.379 (0.03)   &  /   &  0.58 (0.026)   &  0.045 (7.85e-03)   &   /   \\ 
         \hline 
       % bernstein basic 
       \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\centering  Bern.}}}              &  DeC  &  0.28 (0.58)   &  0.025 (0.153)   &  0.074 (0.078)   &  0.455 (0.078)   &  0.025 (5.46e-03)   &  0.017 (0.04)   \\ 
               &  SSPRK  &  0.546 (0.127)   &  0.403 (0.058)   &  0.298 (0.012)   &  0.546 (0.026)   &  0.403 (1.73e-03)   &  0.298 (3.57e-04)   \\ 
               &  RK  &  0.298 (0.127)   &  0.298 (0.026)   &  0.22 (0.026)   &  0.403 (0.012)   &  0.298 (1.73e-03)   &  0.22 (3.57e-04)   \\ 
         \hline 
        \end{tabular} 
    \end{center} 
     \caption{\textit{T} mesh: Optimized CFL and penalty coefficient $\delta $ in parenthesis, minimizing $\eta_u$. \newline
     $^*$ These values are dangerous, cf \ref{sec:fourier_rocket}.   } \label{tab:dispersion_cfl_LinearAdvection_meshT-RES}
 \end{table}%

==> convergence_tab_meshcombined_nlsw_2D-unsteady_case_tf01_old.tex <==
\begin{table}[H] 
\small  
 \begin{center} 
		\begin{tabular}{| c | c || c | c | c || c | c | c | }  
	     \hline 
	     \multicolumn{2}{|c||}{Element $\&$ }  & \multicolumn{3}{|c||}{OSS}  & \multicolumn{3}{|c|}{CIP}  \\ \hline 
	     \multicolumn{2}{|c||}{ Time scheme }  & $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$   & $\mathbb{P}_1$ & $\mathbb{P}_2$ & $\mathbb{P}_3$  \\ \hline \hline 
       % lagrange basic 
Basic              &  SSPRK & 2.34 & 2.68 & 3.86 & 1.94 & 2.53 & 3.61 \\ 
         \hline 
       % lagrange cubature 
       \multirow{2}{*}{\centering  Cub.}               &  SSPRK & 2.03 & 3.13 & 3.57 & 1.74 & 2.7 &  /  \\ 
               &  DeC & 2.13 & 3.09 & 3.57 & 1.71 & 2.7 &  /  \\ 
         \hline 
       % bernstein basic 
Bern.              &  DeC & 2.33 & 3.19 & 2.87 & 1.75 & 2.77 & 2.76 \\ 
         \hline 
        \end{tabular} 
    \end{center} 
     \caption{Summary tab of convergence order, unsteady vortex, $t_f=0.1s$.\newline
     \textit{"/"} means that the scheme is clearly unstable. } \label{tab:conv_order_nlsw_2D-unsteady}
\end{table}%

==> numerical_longtime.tex <==
\subsection{Long time simulation - shallow water system}
For a last numerical test, we consider again the non linear shallow water benchmark, i.e. the one define in the section \ref{sec:nlsw2D_results-meshX}, but on a domain $\Omega = [0,20] \times [0,1]$ and $t_f =25s$. Which correspond to a travelling vortex in a long free surface flow (see \ref{fig:travelling_vortex} for $\Omega = [0,2] \times [0,1]$ and $t_f=1s$). An extension of this test case was developed by M. Ricchiuto and D. Torlo in \cite{ricchiuto2021analytical} for Euler equations. \\
\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{image_element/travelling_vortex2Davide_longbathy.png}
\caption{Initial water elevation - Travelling vortex test case, $\Omega = [0,20] \times [0,1]$ and $t_f =25s$.} \label{fig:travelling_vortex}
\end{figure}

We will compare the most relevant numerical methods that we obtained in the last section in term of accuracy and cpu time. 
We consider:
\begin{itemize}
	\item $\TP_2$ and $\TP_3$ \textit{cubature} discretizations with the OSS stabilization technique and SSPRK time scheme.
	\item $\P_2$ and $\P_3$ \textit{basic} discretizations with the OSS stabilization technique and SSPRK time scheme.
\end{itemize}

\begin{table}[H] 
\small  
\begin{center} 
  \begin{tabular}{| c | c || c | c | c | c | }  
    \hline 
    \multicolumn{2}{|c||}{Element $\&$ }  & \multirow{2}{*}{number of nodes} & \multirow{2}{*}{CFL} & \multirow{2}{*}{Error norm $L_1$} & \multirow{2}{*}{cpu-time $(s)$} \\ % time to download the grid and initialise matrices
    \multicolumn{2}{|c||}{ Time scheme }  & & &  & \\ \hline \hline 
    %
    % lagrange basic 
    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering  Basic}}} \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering  SSPRK}}} & \multirow{2}{*}{$\P_2$} & \multirow{2}{*}{10917} & \multirow{2}{*}{0.2 } & \multirow{2}{*}{4.575e-4}  & \multirow{2}{*}{24783 } \\ % 35.30256128311157
    & & &  &   &   \\ \cline{3-6} % 
    %
    & \multirow{2}{*}{$\P_3$} &  \multirow{2}{*}{11386} & \multirow{2}{*}{0.22 } & \multirow{2}{*}{3.514e-4 } & \multirow{2}{*}{19220 } \\ % 78.38076543807983
    & & &  &   &  \\ \hline \hline % 
    %
    % lagrange cubature 
    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering  SSPRK}}} & \multirow{2}{*}{$\TP_2$} & \multirow{2}{*}{16165} & \multirow{2}{*}{0.2 } &  \multirow{2}{*}{4.107e-4}  & \multirow{2}{*}{10966 } \\ % 17.678476333618164
    & & &  &   &  \\ \cline{3-6} % 240.6811318397522
    %
    &  \multirow{2}{*}{$\TP_3$} &  \multirow{2}{*}{16258} & \multirow{2}{*}{ 0.025} &\multirow{2}{*}{ 4.876e-4}  & \multirow{2}{*}{40417 } \\ % 21.43336844444275
    & & &  &   &  \\ \hline %
  \end{tabular} 
\end{center} 
\caption{Summary tab of numerical tests. At left: the numerical schemes, at right: results.} 
\end{table}%

For the same mesh between \textit{Basic} and \textit{Cubature} elements, and the approximately same number of nodes between elements of order 2 and 3, there are two important things to notice. First of all, the error is approximately the same for the fourth methods. \\
Secondly, regarding the cpu-time, we observe that $\TP_3$ elements is much more expensive than others methods, which can be explain by the very low CFL number (ten times lower). Then, for approximatly the same CFL number, the $\TP_2$ discretization is the best choice for this numerical test. Indeed, it is twice more cheaper in term of time of computation, which can be explain by the mass matrix inversion which does not appear in this method. 



%\begin{table}[H] 
%\small  
%\begin{center} 
%  \begin{tabular}{| c | c || c | c | c | }  
%    \hline 
%    \multicolumn{2}{|c||}{Element $\&$ }  & \multirow{2}{*}{number of nodes} & \multirow{2}{*}{Error norm $L_1$} & \multirow{2}{*}{cpu-time $(s)$} \\ % time to download the grid and initialise matrices
%    \multicolumn{2}{|c||}{ Time scheme }  & & &   \\ \hline \hline 
%    %
%    % lagrange basic 
%    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering  Basic}}} \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering  SSPRK}}} & \multirow{2}{*}{$\P_2$} & \multirow{2}{*}{10917} & \multirow{2}{*}{4.575e-4}  & \multirow{2}{*}{24782.893170833588} \\ % 35.30256128311157
%    & &   &   &   \\ \cline{3-5} % 
%    %
%    & \multirow{2}{*}{$\P_3$} &  \multirow{2}{*}{11386} & \multirow{2}{*}{3.514e-4 } & \multirow{2}{*}{19220.445920228958} \\ % 78.38076543807983
%    & &   &   &  \\ \hline \hline % 
%    %
%    % lagrange cubature 
%    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering  Cub.}}} \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering  SSPRK}}} & \multirow{2}{*}{$\TP_2$} & \multirow{2}{*}{16165} &  \multirow{2}{*}{4.107e-4}  & \multirow{2}{*}{10966.401886463165} \\ % 17.678476333618164
%    & &   &   &  \\ \cline{3-5} % 240.6811318397522
%    %
%    &  \multirow{2}{*}{$\TP_3$} &  \multirow{2}{*}{16258} &\multirow{2}{*}{ 4.876e-4}  & \multirow{2}{*}{40417.3354511261} \\ % 21.43336844444275
%    & &   &   &  \\ \hline %
%  \end{tabular} 
%\end{center} 
%\caption{Summary tab of numerical tests. At left: the numerical schemes, at right: results.} 
%\end{table}%
